KILT: a Benchmark for Knowledge Intensive Language Tasks

Challenging problems such as open-domain question answering, fact checking, slot filling and entity linking require access to large, external knowledge sources. While some models do well on individual tasks, developing general models is difficult as each task might require computationally expensive indexing of custom knowledge sources, in addition to dedicated infrastructure. To catalyze research on models that condition on specific information in large textual resources, we present a benchmark for knowledge-intensive language tasks (KILT). All tasks in KILT are grounded in the same snapshot of Wikipedia, reducing engineering turnaround through the re-use of components, as well as accelerating research into task-agnostic memory architectures. We test both task-specific and general baselines, evaluating downstream performance in addition to the ability of the models to provide provenance. We find that a shared dense vector index coupled with a seq2seq model is a strong baseline, outperforming more tailor-made approaches for fact checking, open-domain question answering and dialogue, and yielding competitive results on entity linking and slot filling, by generating disambiguated text. KILT data and code are available at https://github.com/facebookresearch/KILT.

==> figures/barplot/bleu/Makefile <==
all:
	gnuplot -c script.gnuplot data/fever.txt && epstopdf chart.eps && rm chart.eps && pdfcrop chart.pdf && rm chart.pdf && mv chart-crop.pdf fever.pdf && \
	gnuplot -c script.gnuplot data/hotpotqa.txt && epstopdf chart.eps && rm chart.eps && pdfcrop chart.pdf && rm chart.pdf && mv chart-crop.pdf hotpotqa.pdf && \
	gnuplot -c script.gnuplot data/nq.txt && epstopdf chart.eps && rm chart.eps && pdfcrop chart.pdf && rm chart.pdf && mv chart-crop.pdf nq.pdf && \
	gnuplot -c script.gnuplot data/triviaqa.txt && epstopdf chart.eps && rm chart.eps && pdfcrop chart.pdf && rm chart.pdf && mv chart-crop.pdf triviaqa.pdf && \
	gnuplot -c script.gnuplot data/wow.txt && epstopdf chart.eps && rm chart.eps && pdfcrop chart.pdf && rm chart.pdf && mv chart-crop.pdf wow.pdf && \
	gnuplot -c script.gnuplot data/zeroshot.txt && epstopdf chart.eps && rm chart.eps && pdfcrop chart.pdf && rm chart.pdf && mv chart-crop.pdf zeroshot.pdf 

==> tables/backups/F1score-test.tex <==
\begin{table*}[h]
\centering

\resizebox{\textwidth}{!}{   

\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{llr@{\hskip 3em}rrrrrrrrr}
 \toprule
% && \multicolumn{4}{l}{\textbf{~~CoarsexGrained}} & \multicolumn{6}{c}{\textbf{FinexGrained}}\\ % SB: Something odd is going on with centering. Fixing manually for now.
\multicolumn{2}{c}{\textbf{Model}} & \textbf{Avg} & \textbf{FE} & \textbf{NQ} & \textbf{HP} & \textbf{TR} & \textbf{ZS} & \textbf{AY} & \textbf{WI} & \textbf{CW} & \textbf{WW}  \\
\midrule
\multicolumn{12}{c}{F1 Score} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{ts}}} & NSMN & - & 66.10 & - & - & - & - & - & - & - & -  \\ 
& BERT +DPR  & - & 69.68 & 44.34 & 17.35 & \textbf{71.26} & \textbf{37.28} & - & - & - & -  \\ 
& BLINK & - & - & - & - & - & - & \textbf{89.71} & \textbf{88.11} & \textbf{78.05} & -  \\ 
& Trans MemNet & - & - & - & - & - & - & - & - & - & 11.5  \\ 
\cmidrule(lr){0-11}
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{im}}} & 
BART-large & 44.91 &  78.93 & 26.67 & 21.97 & 19.91 & 14.4 & 88.31 & 71.52 & 70.32 & 12.17 \\

& T5-base & 43.39 & 76.29 & 25.28 & 19.57 & 15.55 & 13.52 & 86.21 & 71.30 & 69.63 & 13.16  \\ 
%& T5-large & x & x & x & x & x & x & x & x & x & x  \\ 
\cmidrule(lr){0-11}
\multirow{1}{*}{\rotatebox[origin=c]{90}{\textit{ex}}} & BART +DPR & \textbf{56.39} & \textbf{86.74} & \textbf{47.29} & \textbf{34.07} & 60.76 & 35.55 & 86.63 & 71.84 & 69.2 & \textbf{15.39} \\
& RAG & x & 78.1 & 45.74 & 36.03 & 63.43 & 49.95 & 85.76 & 71.66 & 68.62 & 12.81 \\
& FiD & - & - & 55.84 & - & - & - & - & - & - & - \\
\midrule
\multicolumn{12}{c}{KILT-F1-score} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{ts}}} & NSMN & - & 41.88 & - & - & - & - & - & - & - & -  \\ 
& BERT +DPR  & - & \textbf{57.97} & \textbf{32.52} & 0.0 & \textbf{34.88} & \textbf{27.09} & - & - & - & -  \\ 
& BLINK & - & - & - & - & - & - & \textbf{81.54} & \textbf{80.24} & \textbf{68.79} & -  \\ 
& Trans MemNet & - & - & - & - & - & - & - & - & - & 2.2  \\ 
\cmidrule(lr){0-11}
\multirow{1}{*}{\rotatebox[origin=c]{90}{\textit{ex}}} & BART +DPR & \textbf{34.86} & 47.68 & 31.13 & \textbf{2.53} & 32.28 & 19.52 & 76.0  &  49.94 &  50.62 & \textbf{4.0} \\
& RAG & x & * & 31.01 & * & * & * & * & * & * & * \\
\bottomrule
\end{tabular}
}
\caption{F1-score and KILT-F1-score on test data. Baselines are grouped by task-specific (\textit{ts}) and general with implicit (\textit{im}) or explicit (\textit{ex}) knowledge access. We don't report KILT-F1-score for \textit{im} baselines since no provenance information is returned by them. }
\label{tab:f1-score-test}
\end{table*}



==> tables/backups/datasets_bak.tex <==
\begin{table*}[t!]
    \centering
\resizebox{\textwidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
    \begin{tabular}{rlcccc}
        \toprule
        \multicolumn{2}{c}{Original dataset} &  Task & Size (train / dev / test)\\
        \midrule
        \textbf{FEV} &FEVER~\cite{Thorne18Fever} & Fact Checking & 104,966 / 10,444 / 10,100 \\
        \textbf{NQ} & Natural Questions~\cite{kwiatkowski2019natural} &  Open Domain QA & 87,372 / 2,837 / 1,444\\
        \textbf{HoPo} & HotpotQA~\cite{yang2018hotpotqa} &  Open Domain QA & 88,869 / 5,600 / 5,569 \\
        \textbf{TQA} & TriviaQA~\cite{joshi2017triviaqa} &  Open Domain QA & 61,844 / 5,359 / 6,586  \\
        \textbf{ELI5} & ELI5\cite{fan2019eli5} &  Open Domain QA & 272,634 / 1,878 / 911 \\
        \textbf{T-REx} & T-REx~\cite{elsahar2019t} & Slot Filling & 2,284,168 / 5,000 / 5,000  \\
        \textbf{zsRE} & Zero Shot RE~\cite{levy2017zero} &  Slot Filling & 147,909 / 3,724 / 4,966  \\
        \textbf{AY2} & AIDA CoNLL-YAGO~\cite{hoffart2011robust} &  Entity Linking  & 18,395 / 4,784 / 4,463  \\
        \textbf{WnWi} & WNED-WIKI~\cite{guo2018robust} &  Entity Linking  & - / 3,396 / 3,376  \\
        \textbf{WnCw} & WNED-CWEB~\cite{guo2018robust} &  Entity Linking  & - / 5,599 / 5,543  \\
        \textbf{WoW} & Wizard of Wikipedia~\cite{dinan2018wizard}  &  Dialogue  & 94,577 / 3,058 / 2,944  \\
        \midrule
        \multicolumn{3}{c}{total} & * / * / * & \\
        \bottomrule
    \end{tabular}
}
    \caption{Datasets and tasks considered in KILT.}
    \label{tab:datasets}
\end{table*}


==> tables/backups/datasets_stats_bak.tex <==
\begin{table*}[t!]
    \centering
\resizebox{\textwidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
    \begin{tabular}{rlllllcccccc}
        \toprule
        & \makecell{input\\format} & \makecell{input\\domain} & \makecell{output\\format} & \makecell{evidence\\level} & \makecell{evidence\\nature} & mutli-hop & \makecell{average\\provenance\\size} & \makecell{average\\provenance\\number} & \makecell{average\\provenance\\pages}  &
        \makecell{average\\answers\\number}  \\
        \midrule
        \textbf{FEV} & claim & Wikipedia & classification & sentence & human annotations & x & 1.12 & 1.35 & 1.13 & 1 \\
        \textbf{NQ} & query & Google Search & extractive & answer + sentence & human annotations & & 1 & 3.22 & 1.57  & 2.08  \\
        \textbf{HoPo} & question & Wikipedia & abstractive & sentence & human annotations & x & 2.4 & 1 & 2 & 1 \\
        \textbf{TQA} & question & Trivia quiz & extractive & answer & distant supervision & & 1 & 3.39 & 1.68 & 28.67  \\
        \textbf{eli5} & long question & reddit & abstractive & sentence & human annotations & & 1 & 1.56 & 1.52 & 4.53   \\
        \textbf{T-REx} & structured & Wikidata  & entity & sentence & distant supervision & & 1 & 1.68 & 1.26 & 5.29   \\
        \textbf{zsRE} & structured & Wikidata & entity &  sentence & human annotations & & 1 & 1 & 1 & 1  \\
        \textbf{AY2} & text chunk & CoNLL & entity  & page & human annotations  & & 1 & 1 & 1 & 1  \\
        \textbf{WnWi} & text chunk & Wikipedia & entity &  page & human annotations & & 1 & 1 & 1 & 1   \\
        \textbf{WnCw} & text chunk & ClueWeb & entity &  page & human annotations   & & 1 & 1 & 1 & 1   \\
        \textbf{WoW} & conversation & chat & abstractive &  sentence & human annotations  & & 1 & 1 & 1 & 1   \\
        \bottomrule
    \end{tabular}
}
    \caption{Datasets characteristics and test stats.}
    \label{tab:datasets}
\end{table*}


==> tables/datasets_joined.tex <==
\clearpage
\begin{table}[t!]
\begin{adjustbox}{angle=90}
%\begin{table*}[t!]
    % \centering
\resizebox{\textheight}{!}{    
    \begin{tabular}{ll|l|llll|ll|lll|l}
    \toprule
    & & \multicolumn{1}{c}{Fact Checking} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{2}{c}{Slot Filling} & \multicolumn{3}{c}{Entity Linking} &  \multicolumn{1}{c}{Dialouge} \\
    & &  \multicolumn{1}{c}{\textbf{FEV}} &  \multicolumn{1}{c}{\textbf{NQ}} &  \multicolumn{1}{c}{\textbf{HoPo}} &  \multicolumn{1}{c}{\textbf{TQA}} &  \multicolumn{1}{c}{\textbf{ELI5}} &  \multicolumn{1}{c}{\textbf{T-REx}} &  \multicolumn{1}{c}{\textbf{zsRE}} &  \multicolumn{1}{c}{\textbf{AY2}} &  \multicolumn{1}{c}{\textbf{WnWi}} &  \multicolumn{1}{c}{\textbf{WnCw}} &  \multicolumn{1}{c}{\textbf{Wow}}\\
    \midrule
    Original Dataset & & FEVER & Natural Questions & HotpotQA & TriviaQA & ELI5 & T-REx & Zero Shot RE & AIDA CoNLL-YAGO & WNED-WIKI & WNED-CWEB & Wizard of Wikipedia\\
    Reference & & \citeauthor{Thorne18Fever} & \citeauthor{kwiatkowski2019natural} & \citeauthor{yang2018hotpotqa}
 & \citeauthor{joshi2017triviaqa} & \citeauthor{fan2019eli5} & \citeauthor{elsahar2019t} & \citeauthor{levy2017zero} & \citeauthor{hoffart2011robust} & \citeauthor{guo2018robust} & \citeauthor{guo2018robust} & \citeauthor{dinan2018wizard}\\
   Year & & 2018 & 2019 & 2018 & 2017 & 2019 & 2019 & 2017 & 2011 & 2018 & 2018 & 2018\\
   % Task & Fact Checking & Open Domain QA & Open Domain QA & Open Domain QA & Open Domain QA & Slot Filling & Slot Filling & Entity Linking & Entity Linking & Entity Linking & Dialogue\\
   \multirow{3}{*}{Size}& Train &  & & & & & & & & &\\
   & Dev & & & & & & & & & & &\\
   & Test & & & & & & & & & & &\\
   Input Format & & Claim & Query & Question & Question & Long Question & Structured & Structured & Text Chunk & Text Chunk & Text Chunck & Conversation\\
   Input Domain & & Wikipedia & Google Search & Wikipedia & Trivia quiz & Reddit & Wikidata & Wikidata & CoNLL & Wikipedia & ClueWeb & Chat\\
   Output Format & & Classification & Extractiv & Abstractive & Extractive & Abstractive & Entity & Entity & Entity & Entity & Entity & Abstractive\\
   Evidence Level & & Sentence & Answer \& Sentence & Sentence & Answer & Sentence & Sentence & Sentence & Page & Page & Page & Sentence\\
   Evidence Nature & & Human & Human & Human & Distant Supervision & Human & Distant Supervision & Human & Human & Human & Human & Human\\
   Multi-hop & & Yes & No & Yes & No & No & No & No & No & No & No & No\\
   \multirow{4}{*}{Average Provenance}& Size & & & & & & & & & & &\\
   & Number & & & & & & & & & & &\\
   & Pages & & & & & & & & & & &\\
   & Answers & & & & & & & & & & &\\
 \bottomrule
    \end{tabular}
}    
% \end{table*}
\end{adjustbox}
\end{table}

\if 0
\begin{table*}[t!]
    \centering
\resizebox{\textwidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
    \begin{tabular}{rlcccc}
        \toprule
        \multicolumn{2}{c}{Original dataset} &  Task & Size (train / dev / test)\\
        \midrule
        \textbf{FEV} &FEVER~\cite{Thorne18Fever} & Fact Checking & 104,966 / 10,444 / 10,100 \\
        \textbf{NQ} & Natural Questions~\cite{kwiatkowski2019natural} &  Open Domain QA & 87,372 / 2,837 / 1,444\\
        \textbf{HoPo} & HotpotQA~\cite{yang2018hotpotqa} &  Open Domain QA & 88,869 / 5,600 / 5,569 \\
        \textbf{TQA} & TriviaQA~\cite{joshi2017triviaqa} &  Open Domain QA & 61,844 / 5,359 / 6,586  \\
        \textbf{ELI5} & ELI5\cite{fan2019eli5} &  Open Domain QA & 272,634 / 1,947 / 1,040 \\
        \textbf{T-REx} & T-REx~\cite{elsahar2019t} & Slot Filling & 2,284,168 / 5,000 / 5,000  \\
        \textbf{zsRE} & Zero Shot RE~\cite{levy2017zero} &  Slot Filling & 147,909 / 3,724 / 4,966  \\
        \textbf{AY2} & AIDA CoNLL-YAGO~\cite{hoffart2011robust} &  Entity Linking  & 18,395 / 4,784 / 4,463  \\
        \textbf{WnWi} & WNED-WIKI~\cite{guo2018robust} &  Entity Linking  & - / 3,396 / 3,376  \\
        \textbf{WnCw} & WNED-CWEB~\cite{guo2018robust} &  Entity Linking  & - / 5,599 / 5,543  \\
        \textbf{WoW} & Wizard of Wikipedia~\cite{dinan2018wizard}  &  Dialogue  & 94,577 / 3,058 / 2,944  \\
        \midrule
        \multicolumn{3}{c}{total} & * / * / * & \\
        \bottomrule
    \end{tabular}
}
    \caption{Datasets and tasks considered in KILT.}
    \label{tab:datasets}
\end{table*}

\begin{table*}[t!]
    \centering
\resizebox{\textwidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
    \begin{tabular}{rlllllcccccc}
        \toprule
        & \makecell{input\\format} & \makecell{input\\domain} & \makecell{output\\format} & \makecell{evidence\\level} & \makecell{evidence\\nature} & mutli-hop & \makecell{average\\provenance\\size} & \makecell{average\\provenance\\number} & \makecell{average\\provenance\\pages}  &
        \makecell{average\\answers\\number}  \\
        \midrule
        \textbf{FEV} & claim & Wikipedia & classification & sentence & human annotations & x & 1.12 & 1.35 & 1.13 & 1 \\
        \textbf{NQ} & query & Google Search & extractive & answer + sentence & human annotations & & 1 & 3.22 & 1.57  & 2.08  \\
        \textbf{HoPo} & question & Wikipedia & abstractive & sentence & human annotations & x & 2.4 & 1 & 2 & 1 \\
        \textbf{TQA} & question & Trivia quiz & extractive & answer & distant supervision & & 1 & 3.39 & 1.68 & 28.67  \\
        \textbf{eli5} & long question & reddit & abstractive & sentence & human annotations & & 1 & 1.56 & 1.52 & 4.53   \\
        \textbf{T-REx} & structured & Wikidata  & entity & sentence & distant supervision & & 1 & 1.68 & 1.26 & 5.29   \\
        \textbf{zsRE} & structured & Wikidata & entity &  sentence & human annotations & & 1 & 1 & 1 & 1  \\
        \textbf{AY2} & text chunk & CoNLL & entity  & page & human annotations  & & 1 & 1 & 1 & 1  \\
        \textbf{WnWi} & text chunk & Wikipedia & entity &  page & human annotations & & 1 & 1 & 1 & 1   \\
        \textbf{WnCw} & text chunk & ClueWeb & entity &  page & human annotations   & & 1 & 1 & 1 & 1   \\
        \textbf{WoW} & conversation & chat & abstractive &  sentence & human annotations  & & 1 & 1 & 1 & 1   \\
        \bottomrule
    \end{tabular}
}
    \caption{Datasets characteristics and test stats.}
    \label{tab:datasets}
\end{table*}


\fi

==> tables/old/EMscore-dev.tex <==
\begin{table*}[t!]
\centering

\resizebox{\textwidth}{!}{   

\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lr@{\hskip 3em}rrrrrrrrr}
 \toprule
% && \multicolumn{4}{l}{\textbf{~~CoarsexGrained}} & \multicolumn{6}{c}{\textbf{FinexGrained}}\\ % SB: Something odd is going on with centering. Fixing manually for now.
\textbf{Model} & \textbf{Avg} & \textbf{FE} & \textbf{NQ} & \textbf{HP} & \textbf{TR} & \textbf{ZS} & \textbf{AY} & \textbf{WI} & \textbf{CW} & \textbf{WW}  \\

\midrule
\multicolumn{11}{c}{EM Score} \\
\midrule

BERT +DPR & - & - & 41.23 & 10.82  & 67.40 & x & - & - & - & -  \\ 


BART-large & 36.28 &  80.67 & 25.23 & 16.86 & 8.83 & 4.97 & 86.94 & 51.06 & 51.96 & 0.0 \\


T5-base & 33.88 & 79.77 & 21.51 & 12.66 & 8.93 & 1.58 & 82.08 & 49.05 & 49.41 & 0.0 \\

BART +DPR & - & 88.11 & 43.78 & 25.75 & 51.58 & 26.78 & 86.64 & 49.97 & 49.97 & - \\
RAG** & - & 80.16 & 44.49 & 27.68 & 58.15 & 47.77 & 77.78 & 51.53 & 50.12 & 0.09 \\
\midrule
\multicolumn{11}{c}{KILT-EM-score} \\
\midrule
BERT +DPR  & - & - & 32.41 & 0.0  & 31.76 & *  & - & - & - & -  \\ 
BART +DPR & - & 48.21 & 29.05 & 1.8 & 29.09 & 21.85 & 2.99 & 0.0 & 0.0 & - \\
%RAG** & - & 0.0 & 16.16 & 1.12 & 19.0 & 16.08 & 0.0 & 0.0 & 0.0 & 0.0 \\
\bottomrule
\end{tabular}
}
\caption{EM score dev}
\label{tab:f1scoredev}
\end{table*}

==> tables/old/EMscore-test.tex <==
\begin{table*}[h!]
\centering

\resizebox{\textwidth}{!}{   

\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lr@{\hskip 3em}rrrrrrrrr}
 \toprule
% && \multicolumn{4}{l}{\textbf{~~CoarsexGrained}} & \multicolumn{6}{c}{\textbf{FinexGrained}}\\ % SB: Something odd is going on with centering. Fixing manually for now.
\textbf{Model} & \textbf{Avg} & \textbf{FE} & \textbf{NQ} & \textbf{HP} & \textbf{TR} & \textbf{ZS} & \textbf{AY} & \textbf{WI} & \textbf{CW} & \textbf{WW}  \\

\midrule
\multicolumn{11}{c}{EM Score} \\
\midrule
BERT +DPR & - & - & 37.0 & 11.29  & 66.79 & 29.06 & - & - & - & -  \\ 
BART-large & 34.99 &  78.93 & 20.4 & 15.37 & 8.35 & 12.03 & 78.09 & 49.02 & 52.72 & 0.0 \\
T5-base & 33.01 & 76.29 & 17.09 & 12.64 & 6.22 & 9.02 & 74.38 & 49.28 & 52.22 & 0.0 \\


BART +DRP & 45.68 &  86.74 & 39.64 & 25.18 & 50.77 & 32.2 & 76.0 & 49.94 & 50.62 & 0.0 \\
RAG  & - & 78.1 & 39.12 & 26.97 & 57.61 & 45.03 & 73.58 & 50.53 & 50.62 & 0.0 \\
FiD & - & - & 47.36 & - & - & - & - & - & - & - \\
\midrule
\multicolumn{11}{c}{KILT-EM-score} \\
\midrule
BERT +DPR  & - & - & 28.51 & 0.0  & 32.99 & 22.61  & - & - & - & -  \\ 
BART +DRP & 13.93 &  47.68 & 27.28 & 1.96 & 27.48 & 18.25 & 1.97 & 0.18 & 0.61 & 0.0 \\
%RAG** & - & 0.0 & 14.67 & 1.08 & 19.16 & 13.49 & 0.0 & 0.0 & 0.0 & 0.0 \\
\bottomrule
\end{tabular}
}
\caption{EM score test}
\label{tab:f1scoredev}
\end{table*}

==> tables/old/F1score-dev.tex <==
\begin{table*}[h!]
\centering

\resizebox{\textwidth}{!}{   

\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lr@{\hskip 3em}rrrrrrrrr}
 \toprule
% && \multicolumn{4}{l}{\textbf{~~CoarsexGrained}} & \multicolumn{6}{c}{\textbf{FinexGrained}}\\ % SB: Something odd is going on with centering. Fixing manually for now.
\textbf{Model} & \textbf{Avg} & \textbf{FE} & \textbf{NQ} & \textbf{HP} & \textbf{TR} & \textbf{ZS} & \textbf{AY} & \textbf{WI} & \textbf{CW} & \textbf{WW}  \\

\midrule
\multicolumn{11}{c}{F1 Score} \\
\midrule
BERT +DPR & - & - & 54.31 & 21.27 & 40.87 & - & - & - & - & - \\

BART-large & 46.41 &  80.67 & 30.58 & 23.81 & 19.79 & 13.75 & 92.99 & 73.32 & 70.24 & 12.61 \\ 

T5-base & 44.49 & 79.77 & 28.92 & 19.73 & 19.22 & 10.80 & 90.15 & 70.54 & 68.26 & 13.09 \\

BART +DPR & - & 88.11 & 50.8 & 35.2 & 61.38 & 36.91 & 92.58 & 72.48 & 68.66 & 14.99 \\
%RAG & - & 80.16 & 51.03 & 37.37 & 64.1 & 57.98 & 87.49 & 72.78 & 68.99 & 13.18 \\
\midrule
\multicolumn{11}{c}{KILT-F1-score} \\
\midrule
BERT +DPR & - & - & 48.17 & 16.96 & 71.46 & - & - & - & - & - \\
BART +DPR & - & 48.21 & 32.27 & 2.23 & 33.59 & 24.21 & 3.23 & 0.0 & 0.0 & - \\
%RAG & - & 0.0 & 18.11 & 1.44 & 20.84 & 18.1 & 0.0 & 0.04 & 0.0 & 2.52 \\
\bottomrule
\end{tabular}

}
\caption{F1-score dev}
\label{tab:f1scoredev}
\end{table*}

==> tables/old/F1score-test.tex <==
\begin{table*}[h]
\centering

\resizebox{\textwidth}{!}{   

\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{llr@{\hskip 2em}rrrrrrrrrrr}
 \toprule
% && \multicolumn{4}{l}{\textbf{~~CoarsexGrained}} & \multicolumn{6}{c}{\textbf{FinexGrained}}\\ % SB: Something odd is going on with centering. Fixing manually for now.
&&& \multicolumn{1}{c}{Fact Check.} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{2}{c}{Slot Filling} & \multicolumn{3}{c}{Entity Linking} & \multicolumn{1}{c}{Dial.}  \\
\multicolumn{2}{c}{Model} & Avg & \textbf{FEV} & \textbf{NQ} & \textbf{HoPo} & \textbf{TQA} & \textbf{ELI5} & \textbf{T-REx} & \textbf{zsRE}  & \textbf{AY2} & \textbf{WnWi} & \textbf{WnCw} & \textbf{WoW}  \\
\midrule
\multicolumn{12}{c}{F1 Score} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{ts}}} & NSMN & - & 66.10 & - & - & - & - & - & - & - & - & - & -  \\ 
& BERT +DPR  & - & 69.68 & 47.09 & 17.35 & 74.41 & * & * & \textbf{37.28} & - & - & - & -  \\ 
& BLINK & - & - & - & - & - & - & - & - & \textbf{89.71} & \textbf{88.11} & \textbf{78.05} & -  \\ 
& Trans MemNet & - & - & - & - & - & - & - & - & - & - & - & 11.5  \\ 
\cmidrule(lr){0-13}
\multirow{2}{*}{\rotatebox[origin=c]{90}{\textit{im}}} & 
BART-large & * &  78.93 & 28.69 & 21.97 & 39.85 & 18.70 & 49.24 & 12.20 & 88.31 & 71.52 & 70.32 & 12.96 \\

& T5-base & * & 76.29 & 27.73 & 19.57 & 27.83 &  * & * & 13.52 & 86.21 & 71.30 & 69.63 & 13.49 \\ 
%& T5-large & x & x & x & x & x & x & x & x & x & x  \\ 
\cmidrule(lr){0-13}
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{ex}}} & BART +DPR & * & \textbf{86.74} & 49.53 & 34.07 & 67.79 &  * & * & 34.47 & 86.63 & 71.84 & 69.2 & \textbf{15.55} \\
& RAG & * & 78.1 & 52.40 & 36.03 & 75.88 &  14.54 & * & 49.95 & 85.76 & 71.66 & 68.62 & 13.22 \\
& FiD + DPR & * & * & 59.42 & * & * &  * & * & * & * & * & * & * \\
\midrule
\multicolumn{12}{c}{KILT-F1-score} \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{ts}}} & NSMN & - & 41.88 & - & - & - & - & - & - & - & - & - & -  \\ 
& BERT +DPR  & - & \textbf{58.58} & 37.58 & 1.3 & 36.28 & * &  * &  \textbf{27.09} & - & - & - & -  \\ 
& BLINK & - & - & - & - & - & - & - & - & \textbf{81.54} & \textbf{80.24} & \textbf{68.79} & -  \\ 
& Trans MemNet & - & - & - & - & - & - & - & - & - & - & - & 2.2  \\ 
\cmidrule(lr){0-13}
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{ex}}} & BART +DPR & \textbf{34.86} & 47.68 & 34.71 & 2.53 & 35.34 & * & * & 20.32 & 75.48  &  45.20 &  46.87 & 4.0 \\
& RAG & * & * & 36.82 & 4.1 & 40.15 & 1.5 & * & 39.91 & * & * & * & 9.01 \\
& FiD + DPR & * & * & 42.45 & * & * & * & * & * & * & * & * & * \\
\bottomrule
\end{tabular}
}
\caption{F1-score and KILT-F1-score on test data. Baselines are grouped by task-specific (\textit{ts}) and general with implicit (\textit{im}) or explicit (\textit{ex}) knowledge access. We don't report KILT-F1-score for \textit{im} baselines since no provenance information is returned by them. }
\label{tab:f1-score-test}
\end{table*}



==> tables/old/retrieval-test.tex <==
\begin{table*}[t]
\centering

\resizebox{\textwidth}{!}{   

\fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{lr@{\hskip 3em}rrrrrrrrr}
 \toprule
% && \multicolumn{4}{l}{\textbf{~~CoarsexGrained}} & \multicolumn{6}{c}{\textbf{FinexGrained}}\\ % SB: Something odd is going on with centering. Fixing manually for now.
\textbf{Model} & \textbf{Avg} & \textbf{FE} & \textbf{NQ} & \textbf{HP} & \textbf{TR} & \textbf{ZS} & \textbf{AY} & \textbf{WI} & \textbf{CW} & \textbf{WW}  \\
\midrule
\multicolumn{11}{c}{R-Precision} \\
\midrule
DrQA Doc. Ret. & 29.33 & 50.85 & 25.55 & 34.14 & 46.37 & 61.24 & 4.08 & 0.41 & 3.93 & \textbf{37.4}  \\
%BM25 & x & x & x & x & x & x & x & x & x & x  \\
DPR & 25.44 &  55.33 & 50.84 & 25.04 & 44.49 & 26.89 & 2.33 & 0.24 & 1.21 & 22.58 \\
DPR +BERT & - & \textbf{72.93} & \textbf{54.76} & 21.46 & 43.4 & 40.11 & - & - &  - & -  \\
BLINK +flair & \textbf{60.77} & 63.67 & 21.17 & \textbf{46.1} & \textbf{65.58} & \textbf{86.15} & \textbf{81.54} & \textbf{80.24} & \textbf{68.79} & 33.71  \\ 
RAG** & x & * & 55.28 & * & * & * & * & * & * & * \\
\bottomrule
\end{tabular}
}
\caption{R-Precision for retrieval baselines on test data. We additionally report the performance after the BERT-based classifier (for FE) or reader (for NQ,HP,TR) re-ranked relevant pages (i.e., DPR +BERT).}
\label{tab:test-retrieval-results}
\end{table*}
